Measurement of High Energy Gamma Rays from 200 MeV to 1 TeV with the Alpha Magnetic Spectrometer on the International Space Station

In this thesis a measurement of the high energy $\gamma$-ray flux between 200 MeV and 1 TeV with the Alpha Magnetic Spectrometer is presented. The Alpha Magnetic Spectrometer (AMS-02) is a multi-purpose particle detector mounted externally on the International Space Station. Although primarily designed for the measurement of charged cosmic rays AMS-02 is capable of measuring high energy $\gamma$-rays in two complementary modes. Two independent analyses are presented in this thesis, one for each of the two modes. The event selection criteria and the associated resolution functions are presented in detail. The effective area is estimated from a full detector Monte-Carlo simulation and corrected for the most important differences between data and simulation. A full sky model for $\gamma$-rays is constructed from diffuse emission predictions and recent $\gamma$-ray source catalogs. A dedicated analysis of Fermi-LAT data is performed to fully enable a detailed comparison with the AMS result. The measured flux of $\gamma$-rays is presented for various parts of the sky, including comparisons with Fermi-LAT data and with the constructed model. The inner galaxy is studied in detail, as an example of a region in which the photon flux is dominated by diffuse emission. The fluxes of several $\gamma$-ray producing sources, including Vela, Geminga and the Crab pulsar are shown. The Geminga pulsar is studied in detail, revealing its pulsed emission of $\gamma$-rays in the AMS-02 data, which allows to measure its frequency of rotation and to estimate its magnetic field strength and age. Finally, AMS-02 observed an outburst of the flaring blazar CTA-102 at the end of 2016.

==> listoffigures.tex <==
% !TeX root = phd.tex

\clearpage
\listoffigures

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "phd"
%%% fill-column: 100
%%% End:

